Interpreting Adaptive Gradient Methods by Parameter Scaling for Learning-Rate-Free Optimization

We address the challenge of estimating the learning rate for adaptive gradient methods used in training deep neural networks. While several learning-rate-free approaches have been proposed, they are typically tailored for steepest descent. However, although steepest descent methods offer an intuitive approach to finding minima, many deep learning applications require adaptive gradient methods to achieve faster convergence. In this paper, we interpret adaptive gradient methods as steepest descent applied on parameter-scaled networks, proposing learning-rate-free adaptive gradient methods. Experimental results verify the effectiveness of this approach, demonstrating comparable performance to hand-tuned learning rates across various scenarios. This work extends the applicability of learning-rate-free methods, enhancing training with adaptive gradient methods.

==> table/cifar_resnet.tex <==
\begin{tabular}{lcc|lcc}
\hline
\multicolumn{3}{l|}{\textit{Steepest descent}}            & \multicolumn{3}{l}{\textit{Adaptive gradient}}            \\ \hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Train loss} & \textbf{Method} & \textbf{Accuracy} & \textbf{Train loss} \\ \hline
\rowcolor[HTML]{C0C0C0} 
SGD             & 66.7              & 0.233               & Adam            & 68.3              & 0.236               \\
SPS             & 65.2              & 0.359               & PS-SPS          & 65.9              & 0.337               \\
-               &                   &                     & COCOB           & 50.1              & 1.666               \\
DoG             & 66.7              & 0.495               & LDoG            & 63.9              & 0.547               \\
                &                   &                     & D-Adapt Adam    & 65.9              & 0.286               \\
D-Adapt SGD     & 65.6              & 0.312               & Prodigy         & 66.4              & 0.221               \\
                &                   &                     & PS-DA-SGD       & 65.8              & 0.305               \\ \hline
\end{tabular}

==> table/cifar_vgg.tex <==
\begin{tabular}{lcc|lcc}
\hline
\multicolumn{3}{l|}{\textit{Steepest descent}}            & \multicolumn{3}{l}{\textit{Adaptive gradient}}            \\ \hline
\textbf{Method} & \textbf{Accuracy} & \textbf{Train loss} & \textbf{Method} & \textbf{Accuracy} & \textbf{Train loss} \\ \hline
\rowcolor[HTML]{C0C0C0} 
SGD             & 64.7              & 0.038               & Adam            & 65.1              & 0.086               \\
SPS             & 0.01              & 5.041               & PS-SPS          & 53.4              & 0.182               \\
-               &                   &                     & COCOB           & 55.1              & 0.771               \\
DoG             & 56.3              & 0.074               & LDoG            & 56.4              & 0.073               \\
                &                   &                     & D-Adapt Adam    & 48.3              & 0.033               \\
D-Adapt SGD     & 0.01              & 4.605               & Prodigy         & 57.8              & 0.019               \\
                &                   &                     & PS-DA-SGD       & 50.6              & 0.009               \\ \hline
\end{tabular}

==> table/rl_sac.tex <==
\begin{tabular}{lcc|lcc}
\hline
\multicolumn{3}{l|}{\textit{Steepest descent}}              & \multicolumn{3}{l}{\textit{Adaptive gradient}}              \\ \hline
\textbf{Method} & \textbf{Hopper-v2} & \textbf{Humanoid-v2} & \textbf{Method} & \textbf{Hopper-v2} & \textbf{Humanoid-v2} \\ \hline
\rowcolor[HTML]{C0C0C0} 
SGD             & 3466 (5/5)         & NaN (0/5)            & Adam            & 3448 (5/5)         & 5527 (5/5)           \\
-               &                    &                      & COCOB           & 3334 (5/5)         & 5337 (5/5)           \\
DoG             & 1050 (0/5)         & \hphantom e475 (0/5)           & LDoG            & 3277 (1/5)         & \hphantom e469 (0/5)            \\
                &                    &                      & D-Adapt Adam    & 3502 (5/5)         & 5504 (3/5)           \\
D-Adapt SGD     & NaN (0/5)          & NaN (0/5)            & Prodigy         & \hphantom e195 (0/5)          & \hphantom e419 (0/5)            \\
                &                    &                      & PS-DA-SGD       & 3497 (5/5)         & 5534 (5/5)           \\ \hline
\end{tabular}

==> table/semseg.tex <==
\begin{tabular}{lcc}
\hline
\textbf{Method} & \textbf{SegNeXt} & \textbf{Swin-T} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Adam            & 41.5             & 44.1            \\
PS-SPS          & 38.9             & 43.8            \\
COCOB           & 3.78             & 17.5            \\
LDoG            & 35.5             & 43.4            \\
D-Adapt Adam    & 30.0             & 41.5            \\
Prodigy         & 32.1             & 42.2            \\
PS-DA-SGD       & 40.8             & 43.9            \\ \hline
\end{tabular}

==> table/ssl.tex <==
\begin{tabular}{lc}
\hline
\textbf{Method} & \textbf{Accuracy} \\ \hline
\rowcolor[HTML]{C0C0C0} 
Adam            & 54.5              \\
PS-SPS          &                   \\
COCOB           &                   \\
LDoG            &                   \\
D-Adapt Adam    &                   \\
Prodigy         &                   \\
PS-DA-SGD       & \textbf{53.2}     \\ \hline
\end{tabular}

==> table/vit.tex <==
\begin{tabular}{lc|lc}
\hline
\multicolumn{2}{l|}{\textit{Steepest descent}} & \multicolumn{2}{l}{\textit{Adaptive gradient}} \\ \hline
\textbf{Method}       & \textbf{Accuracy}      & \textbf{Method}  & \textbf{Accuracy}  \\ \hline
\rowcolor[HTML]{C0C0C0} 
SGD                   & -                      & Adam             & 75.4               \\
SPS                   &                        & PS-SPS           & 24.0               \\
-                     &                        & COCOB            & 0.14               \\
DoG                   &                        & LDoG             & 0.77               \\
                      &                        & D-Adapt Adam     & 72.4               \\
D-Adapt SGD           & 4.29                   & Prodigy          & 74.6               \\
                      &                        & PS-DA-SGD        & 74.5               \\ \hline
\end{tabular}
